Unsupervised Natural Language Inference via Decoupled Multimodal Contrastive Learning

We propose to solve the natural language inference problem without any supervision from the inference labels via task-agnostic multimodal pretraining. Although recent studies of multimodal self-supervised learning also represent the linguistic and visual context, their encoders for different modalities are coupled. Thus they cannot incorporate visual information when encoding plain text alone. In this paper, we propose Multimodal Aligned Contrastive Decoupled learning (MACD) network. MACD forces the decoupled text encoder to represent the visual information via contrastive learning. Therefore, it embeds visual knowledge even for plain text inference. We conducted comprehensive experiments over plain text inference datasets (i.e. SNLI and STS-B). The unsupervised MACD even outperforms the fully-supervised BiLSTM and BiLSTM+ELMO on STS-B.

==> related.tex <==
\section{Related Work}

{\bf Unsupervised Natura Language Representation Learning} Unsupervised learning has become a new paradigm for natural language representation learning~\cite{devlin2018bert,peters2018deep,radford2019language}. On many NLP tasks, using unsupervised learning as pre-training has achieved state-of-the-art results~\cite{joshi2019spanbert,wang2018glue}. Recent related researches includes the use of larger unsupervised datasets and larger network structures to improve model performance~\cite{raffel2019exploring,DBLP:journals/corr/abs-1907-11692}. Other studies use knowledge distillation~\cite{sun2019patient} or adversarial learning~\cite{clark2020electra} to compress model parameters or accelerate model training.

The success of these efforts has undoubtedly led to the use of self-supervised learning for multimodal learning in this paper. We emphasize that multimodal learning is essential for more accurate understanding of text by representing its visual context. Besides, the pre-trained unsupervised learning model (e.g. BERT~\cite{devlin2018bert}) is used for the parameter initialization of the text encoder in this paper.

{\bf Multimodal Pre-training} Recently, some studies~\cite{li2019unicoder,li2019visualbert} have extended unsupervised natural language representation learning to the multimodal settings, including image~\cite{li2019unicoder,li2019visualbert}, and video~\cite{sun2019videobert}. Due to the great success of BERT, these studies often follow its parameters and network architecture. \cite{lu2019vilbert} uses a co-attention transformer layer to extend the standard transformer layer~\cite{vaswani2017attention}. This new network architecture uses two joint transformers to simultaneously model visual and linguistic features. \cite{li2019unicoder} further treats visual elements and text elements as one sequence, and directly uses a standard transformer to model its joint representation, and uses cloze tasks for joint representation learning.

However, these studies have two problems in solving the problems raised in this paper. First, in their models, the encoders of language features and visual features are coupled. This limits that the downstream tasks of the model must also be multimodal problems. But we want to solve the plain text inference problems. In contrast, the language feature encoder proposed in this paper is decoupled and encode the plain text along. Second, the training of these models only considers text-visual joint task training, which leads to catastrophic forgetting when reasoning over the natural language. In this paper, we propose the lifelong learning regularization to anchor the natural language. In this way we avoid the catastrophic forgetting problem when learning new visual knowledge.

{\bf Self-supervised Learning via Contrastive Learning} Self-supervised learning~\cite{de1994learning,xie2016unsupervised,bojanowski2017unsupervised} is widely used in tasks such as unsupervised image classification, temporal prediction~\cite{goroshin2015unsupervised}, and image inpainting~\cite{huang2014image}. Contrastive learning has become a popular toolkit for this problem. Its core idea is to learn the representation to reconstruct of identify some part of the data. Recently, this goal was formalized to maximize mutual information between different pieces of information~\cite{hjelm2018learning,tian2019contrastive}. Because the mutual information is intractable, some approximations have been proposed, including Noise-Contrastive Estimation~\cite{oord2018representation}, Donsker-Varadhan estimator~\cite{donsker1983asymptotic,hjelm2018learning}, and Jensen-Shannon estimator~\cite{nowozin2016f,hjelm2018learning}.

Although these studies have not been directly applied to the multi-modal data of text2image, some studies also focus on the multimodal data~\cite{hjelm2018learning,tian2019contrastive}. However, their inference of text and other modalities are coupled, which makes it infeasible to represent text with visual knowledge when only text is used as input.


%consider the structured correlations between different modalities, and often treat the data of different modalities as some orthogonal views. Since our problem is for self-supervised learning over text2image data, their matchings have a typical structured relationship~\cite{xu2018attngan}. We need to propose new algorithms to carefully deal with the structural correlations.


